Game Plot Design with an LLM-powered Assistant: An Empirical Study with Game Designers

We introduce GamePlot, an LLM-powered assistant that supports game designers in crafting immersive narratives for turn-based games, and allows them to test these games through a collaborative game play and refine the plot throughout the process. Our user study with 14 game designers shows high levels of both satisfaction with the generated game plots and sense of ownership over the narratives, but also reconfirms that LLM are limited in their ability to generate complex and truly innovative content. We also show that diverse user populations have different expectations from AI assistants, and encourage researchers to study how tailoring assistants to diverse user groups could potentially lead to increased job satisfaction and greater creativity and innovation over time.

==> 5-findings.tex <==
\section{Findings}
\label{sec:findings}
In our post-study questionnaire, we collected both quantitative ratings and qualitative feedback from designers. This approach allowed us to gather detailed insights into their experiences and opinions on the tool.

\subsection{Quantitative Feedback}
\input{Figures/fig_gameroom_features}
We asked game narrative designers to rate their control and ownership over the generated game story and plot in the design room on a scale from 1 to 5. On average, this aspect received a score of 4.5, with 13 out of 14 participants rating it 4 or higher, and no ratings below 3. When evaluating how well the AI system helped improve their game story, the average rating was 4 out of 5, with all responses above 3. Satisfaction with the generated game plot also averaged 4 out of 5, with all ratings exceeding 3.

We also explored which features participants found most valuable in the game room.  As shown in Fig. \ref{fig_gameroom_features}, 12 out of 14 participants favored the \textit{ability to change the game plot during the test session}. \textit{The NPC hidden states dropdown (NPC summary)} and 
\textit{multiplayer setup} in the game room were each favored by 7 out of 14 participants, while feedback features were selected by 6 out of 14. Overall, participants rated the usefulness of the game room for testing with players highly, with 13 out of 14 giving ratings of 4 or 5, resulting in an average score of 4.21.

\subsection{Qualitative Feedback}
This section presents key feedback from game designers and narrative writers on \ourtool{}. Participants highlighted valuable features, suggested improvements, and assessed the AI's strengths and weaknesses. The responses, organized into recurring themes, provide insights into the \ourtool{}'s usability, adaptability, and potential for collaborative game story creation.

\subsubsection{What 1-3 features in \ourtool{} do you find most valuable and would like to see retained?}


Feedback from game designers revealed several features of \ourtool{} that stood out for their flexibility, control, and ease of use in narrative design. A key theme that emerged was \ourtool{}'s adaptability and control in story generation in the Design Room. Designers consistently emphasized how the ability to modify elements such as NPC moods, environments, and plot details allowed them to directly influence AI-generated responses. Answering to the question, one participant noted, ``\textit{The ability to go back and change the mood or environment and have it adapt future responses.}'', while another added, ``\textit{The chance of creating new NPCs, changing the story, and defining everything from personas to thoughts.}'' This dynamic adaptability proved to be a strong draw for users who sought control over the narrative direction.

In the Game Room, the ability to maintain immersion while exercising narrative control was equally appreciated. Designers spoke highly of the ``Wizard of Oz'' setup, which enables game masters to control NPC interactions and adjust the plot without disrupting the players' experience. As one participant explained, ``\textit{The ability to control NPC interactions and tweak narratives without breaking immersion was a strong point, especially with the `Wizard of Oz' setup.}'' Another emphasized the value of flexibility, sharing, ``\textit{The feature of being able to undo and recreate the plot if you see the players aren't enjoying it.}'' This level of control was seen as essential for crafting engaging and responsive game narratives.

Ease of use and collaborative features also surfaced as important strengths. Participants appreciated the simplicity of the user interface, describing it as intuitive and easy to navigate. One designer remarked, ``\textit{The easy-to-understand interface}'', while another highlighted the collaborative potential of the tool, noting, ``\textit{Inviting more people to the room might be very helpful for better collaborations}''. The ability to involve multiple users in testing and design further enhanced the tool's appeal, particularly in group-based design scenarios.

In summary, game designers valued \ourtool{} for its adaptability, control over narrative elements, and support for collaboration. These features contribute to its effectiveness across a wide range of game types and narrative structures, making it a versatile tool for narrative game development.

\subsubsection{Can you identify 1-3 areas for improvement in the GamePlot user interface, or suggest any additional features that would make collaboration easier for you?}

Participants provided several thoughtful suggestions for improving the user interface and enhancing the collaborative experience within \ourtool{}. A recurring theme was the desire for more robust control during the story generation process. Many participants expressed interest in features that could offer more creative input during the design phase. One participant proposed the introduction of mood suggestions for an entire scene, explaining, ``\textit{Mood suggestions for the entire scene (i.e., dev says they want a somber feel for the scene, and the AI adapts the script accordingly).}'' Another participant emphasized the value of exploring multiple plot paths, stating, ``\textit{I'd love to present a few options of how the plot might go down during the design phase.}'' These suggestions reflect a broader interest in having more adaptive and scenario-specific generation tools.

Clarity and organization in the Design Room were also highlighted as areas for improvement. Few participants felt that the current interface could become cluttered, particularly when managing multiple characters or plot elements. One participant remarked, ``\textit{It feels like having everything in one text box could be messy… maybe there should be more features where each NPC has its own text box.}'' another noted that the point of view of NPCs could be clearer, ``\textit{Point of view could be clearer for the user... I wanted the player to be another character that I could add tags to.}'' These comments suggest a need for a more structured interface that clearly distinguishes between different NPCs and narrative components.

The integration of chat features was another focal point for feedback. Some participants recommended separating the in-game chat from the gameplay window to avoid distractions. As one participant suggested, ``\textit{Instead of having /chat inside the game, maybe there should be a chat box off to the side so it doesn't distract the gameplay.}''. Finally, participants expressed enthusiasm for features that could enhance world-building, specifically the ability to generate images based on AI interpretations of visual descriptions. This would allow designers to visualize characters and environments more vividly, supporting the creative development of game worlds.

Overall, participants identified several key areas for improvement, including enhanced customization in story generation, clearer organization in the user interface, expanded game designer controls, and the integration of visual elements to support immersive world-building.





\subsubsection{What are the main weaknesses of the AI model?}

One major issue raised was the LLM's difficulty in maintaining tension and handling multiple conflicts simultaneously. This was a significant drawback for those expecting more complex narrative structures. As one participant explained, ``\textit{It does not have the best grasp on tension balance, or on having multiple conflicts at the same time.}'' The inability to manage tension consistently across different narrative threads limited the LLM's ability to produce more gripping or layered stories. Linearity and predictability of LLM-generated narratives were also questioned. Echoing previous findings from related studies, participants described the AI's responses as often straightforward and uninspired \cite{chakrabarty2023creativity}, lacking the creativity and surprise that make for more compelling storytelling. One participant commented, ``\textit{Obvious answers. No surprise or engagement effect}'', while another added, ``\textit{It is a bit linear, so it seems unlikely that AI will come up with something really unique and interesting}''. This lack of narrative complexity was seen as a significant limitation, especially for those seeking unexpected or novel plot developments.

Concerns were also raised about the quality of the AI's dialogue. Participants noted that the dialogue often lacked depth and failed to capture the nuance of human conversation. One participant expressed doubts, saying, ``\textit{I do have some concerns on whether or not the AI is capable of producing dialogue that sounds natural}'', while another remarked, ``\textit{The AI can be a little straightforward in its narrative... looking for more intriguing narratives.}''

Consistency emerged as another problem, with participants reporting that the AI sometimes failed to maintain plot coherence. Key details could be forgotten or the narrative could veer off track, disrupting the story's internal logic. As one participant described, ``\textit{Sometimes it could be randomized that it doesn't follow original ideas and could go off track}''. 

Finally, participants pointed out usability challenges, particularly with regard to maintaining creative flow. The need to input tags during the writing process was seen as an interruption, making it harder for writers to stay in the "flow state" necessary for smooth, continuous creative work. One participant expressed this frustration, saying, ``\textit{As a writer, I want to remain in a `flow state.' Having to enter tags slows me down.}'' This disruption to the user experience was a notable drawback for those seeking a seamless creative process.

In summary, while the AI model shows potential in story generation, it faces several challenges related to tension management, narrative depth, dialogue quality, consistency, and overall usability, especially for narrative writers aiming for more complex and engaging stories.




==> Figures/fig_gameroom_designer.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=\columnwidth]{Figures/2.Game Room-Designer View.png}
    \caption{Game Room-Designer View}
    \label{fig_gameroom_designer}
\end{figure}

==> Figures/fig_gameroom_player.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=\columnwidth]{Figures/3.Game Room-Player View.png}
    \caption{Game Room-Player View}
    \label{fig_gameroom_player}
\end{figure}
